Availability and Reliability of Wireless Links in 5G Systems: A Space-Time Approach

Wireless links are characterized by fluctuating quality leading to variable packet error rates which are orders of magnitude higher than the ones of wired links. Therefore, it is of paramount importance to investigate the limitations of using 5G wireless links for internet of things (IoT) applications. 5G wireless links in IoT need to assure determinism of process flows via realtime communication anytime and anywhere, which is an utmost requirement for multiple verticals like automotive, industrial automation and aerospace. Based on a space-time approach, in this work, we provide novel definitions of wireless link availability and reliability, assuming a number of access points (APs) and end points (EPs) deployed over a fixed area. Our objective is to analyze the availability of a service in both domains. In the space domain, we characterize spatially available areas consisting of all locations that meet a performance requirement with confidence. In the time domain, we propose a channel allocation scheme accounting for the spatial availability of a cell. To emphasize the incurred space-time performance trade-offs, numerical results are presented, also highlighting the effect of different system parameters on the achievable link availability and reliability.

==> simulation_results/figures/results_spatialanalysis/As_VarThetaAlpha.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%

\begin{tikzpicture}

\begin{axis}[%
width=1.5in,
height=2in,
at={(0.758in,0.481in)},
scale only axis,
xmin=-5,
xmax=5,
xlabel style={font=\color{white!15!black}},
xlabel={$\theta$},
ymin=0.4,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={$\text{A}_\text{s}$},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
-5	0.94263058175714\\
-4.5	0.922622976348299\\
-4	0.916488366661976\\
-3.5	0.890284629101154\\
-3	0.861802644920991\\
-2.5	0.841433596737875\\
-2	0.814518165945886\\
-1.5	0.786783280772089\\
-1	0.771646177695511\\
-0.5	0.754927151609685\\
0	0.712881341011948\\
0.5	0.704688987626541\\
1	0.681302344774229\\
1.5	0.660772216651139\\
2	0.638261640428157\\
2.5	0.615645078165174\\
3	0.594360252089008\\
3.5	0.570438106190981\\
4	0.571342047169509\\
4.5	0.543360787627269\\
5	0.519663640490661\\
};
\addlegendentry{$\alpha\text{ = 0.8}$}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
-5	0.806126700719573\\
-4.5	0.780943041099904\\
-4	0.739460807729894\\
-3.5	0.732282192466415\\
-3	0.70059102934943\\
-2.5	0.684957700589292\\
-2	0.66988147261415\\
-1.5	0.643338253045107\\
-1	0.617362314382072\\
-0.5	0.608624196883369\\
0	0.584973672533399\\
0.5	0.573963888598148\\
1	0.543029594232055\\
1.5	0.54083968902999\\
2	0.510449629894935\\
2.5	0.487846771632426\\
3	0.474680719053595\\
3.5	0.458932703650898\\
4	0.461573746083171\\
4.5	0.441396269340117\\
5	0.427800686961215\\
};
\addlegendentry{$\alpha\text{ = 0.9}$}

\addplot [color=mycolor3, line width=2.0pt]
  table[row sep=crcr]{%
-5	0.989912246916511\\
-4.5	0.984956756573039\\
-4	0.974733641317858\\
-3.5	0.96215535626921\\
-3	0.949302598264665\\
-2.5	0.931742387986592\\
-2	0.911312217530073\\
-1.5	0.897845825589445\\
-1	0.868943752253438\\
-0.5	0.851399452153115\\
0	0.828514061164784\\
0.5	0.796457963601667\\
1	0.781281697941875\\
1.5	0.754066236368085\\
2	0.739799664998043\\
2.5	0.707666327250761\\
3	0.690052539725699\\
3.5	0.672756404009255\\
4	0.644491819091819\\
4.5	0.624225547816028\\
5	0.601964098417615\\
};
\addlegendentry{$\alpha\text{ = 0.7}$}

\addplot [color=green, line width=2.0pt]
  table[row sep=crcr]{%
-5	0.997971650252373\\
-4.5	0.994777533681512\\
-4	0.994470787861432\\
-3.5	0.991961319550386\\
-3	0.984780583329467\\
-2.5	0.974357218572314\\
-2	0.964982207053437\\
-1.5	0.947712210168813\\
-1	0.937654987261411\\
-0.5	0.918883131218135\\
0	0.902734180177219\\
0.5	0.885751369260102\\
1	0.864834784376485\\
1.5	0.836800492659258\\
2	0.808490601069798\\
2.5	0.78907154232111\\
3	0.761269394690258\\
3.5	0.738434425878313\\
4	0.71563968096804\\
4.5	0.713664020559486\\
5	0.670912347383781\\
};
\addlegendentry{$\alpha\text{ = 0.6}$}

\addplot [color=black, line width=2.0pt]
  table[row sep=crcr]{%
-5	1\\
-4.5	0.99997636808317\\
-4	0.999898857974701\\
-3.5	0.999854431756426\\
-3	0.99910615311615\\
-2.5	0.998629925171513\\
-2	0.998682503496733\\
-1.5	0.995973158114521\\
-1	0.991558572048302\\
-0.5	0.987010798954721\\
0	0.982795337278385\\
0.5	0.973933561523014\\
1	0.965033973009595\\
1.5	0.951546071773789\\
2	0.933921723798541\\
2.5	0.918286506179931\\
3	0.904341136049079\\
3.5	0.886296445174088\\
4	0.859719420109754\\
4.5	0.835919609125586\\
5	0.810259734862625\\
};
\addlegendentry{$\alpha\text{ = 0.4}$}

\end{axis}
\end{tikzpicture}%
